Computational predictions of weld structural integrity in hydrogen transport pipelines

We combine welding process modelling with deformation-diffusion-fracture (embrittlement) simulations to predict failures in hydrogen transport pipelines. The focus is on the structural integrity of seam welds, as these are often the locations most susceptible to damage in gas transport infrastructure. Finite element analyses are conducted to showcase the ability of the model to predict cracking in pipeline steels exposed to hydrogen-containing environments. The validated model is then employed to quantify critical H$_2$ fracture pressures. The coupled, phase field-based simulations conducted provide insight into the role of existing defects, microstructural heterogeneity, and residual stresses. We find that under a combination of deleterious yet realistic conditions, the critical pressure at which fracture takes place can be as low as 15 MPa. These results bring new mechanistic insight into the viability of using the existing natural gas pipeline network to transport hydrogen, and the computational framework presented enables mapping the conditions under which this can be achieved safely.

==> pre_commands.tex <==
\usepackage{float,appendix,multicol}
\usepackage[utf8]{inputenc}    % utf8 support       %!!!!!!!!!!!!!!!!!!!!
\usepackage[T1]{fontenc} 
\usepackage{amsmath,amssymb, mathtools,mathrsfs,stmaryrd,titletoc}


% bibtex 
% \usepackage{natbib}
\usepackage[numbers]{natbib}
% \biboptions{sort&compress} %To make [1,2,3] be [1-3]
\usepackage[retainorgcmds]{IEEEtrantools}
\usepackage[usenames]{color}
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{psfrag}
\usepackage[font=small,labelfont=md]{caption,subfig}
\usepackage{multirow}
\usepackage[T1]{fontenc} % typing french                        
\usepackage[bookmarks=true,colorlinks=true,linkcolor=blue,citecolor=red]{hyperref}
\usepackage{float}         % make new float environment such as boxes (captioned)
\usepackage{listings}      % insert source code   
%\usepackage{mathbf}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage{verbatim}
\usepackage{numprint}


% the following packages just to improve the latex experience 
%\usepackage{silence} %
\usepackage{silence}
\WarningsOff\usepackage{siunitx}
\usepackage[norefs,nocites,ignoreunlbld]{refcheck} % warning for unreferred figs/tables/equas
% search in the .log file for unused fig to detect figures not referred to in the text.
\usepackage[activate={true,nocompatibility},final,tracking=true,kerning=true,spacing=true,factor=1100,stretch=10,shrink=10]{microtype}

\captionsetup[figure]{name={Fig.},labelsep=period}

\usepackage[capitalise]{cleveref} %Basically, cleveref must be loaded last.
% clever ref: instead of Fig.~\ref{d}, use \cref{d} or \Cref{d}  capitalise -> Figure 1
% cleverref package
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\crefname{section}{Section}{Sections}
% \crefrange{eq1}{eq5}
\usepackage[textsize=tiny]{todonotes}
\usepackage{nicefrac} % type inline fractions: \nicefrac{1}{2}
\usepackage{setspace}
\usepackage{lineno}  % write numbers for lines
%\usepackage[mediumspace,mediumqspace,Grey,squaren]{SIunits}
\usepackage{totcount} % to count the total number of references and other things
\usepackage[figure,table]{totalcount}
\usepackage{blkarray, bigstrut} % write complicated matrices with borders, see http://mirror.lagoon.nc/pub/ctan/macros/latex/contrib/blkarray/blkarray.pdf
\usepackage{setspace}
\usepackage{tikz}
\usetikzlibrary{arrows,decorations.pathmorphing,decorations.pathreplacing,backgrounds,positioning,fit,matrix,math,shapes.misc}
\tikzset{cross/.style={cross out, draw=black, minimum size=2* (#1-\pgflinewidth), inner sep=0pt, outer sep=0pt}, cross/.default={1pt}}
\usepackage{wasysym}
\usepackage{gensymb} % for degree symbol
\usepackage[section]{placeins} % to place all figures before a new section

% circled text
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=1pt] (char) {#1};}}

% norm ||x||
\newcommand{\normn}{\left|\left| \cdot \right|\right|}
\newcommand{\norm}[1]{\left|\left|#1\right|\right|}

% McAuley brackets <x>
\newcommand{\mcauley}[1]{\langle #1 \rangle}
\usepackage{xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\etc}{\textit{etc.}\@\xspace}
\newcommand{\trace}{\mathrm{tr}}
\newcommand{\bfsigma}{\boldsymbol{\sigma}}
\newcommand{\bfepsilon}{\boldsymbol{\varepsilon}}
\newcommand{\bfu}{\boldsymbol{u}}
\newcommand{\bfx}{\boldsymbol{x}}
\newcommand{\dd}{\mathrm{d}}
\newcommand*{\vd}[3][]{\dfrac{\mathrm{d}^{#1} #2}{\mathrm{d} #3^{#1} }}                          
\newcommand*{\pd}[3][]{\dfrac{\partial^{#1} #2}{\partial #3^{#1} }}  


%--- Box in latex ----
\usepackage{setspace}
\usepackage[many]{tcolorbox}% http://ctan.org/pkg/tcolorbox
\tcbuselibrary{skins,breakable}
\definecolor{mycolor}{rgb}{0.122, 0.435, 0.698}% Rule colour
\newtcolorbox[auto counter,crefname={Box}{Boxes}]{MyBox}[2][]{%
  colback=gray!5!white,colframe=red!75!black,fonttitle=\bfseries,before skip=20pt plus
  2pt,after skip=20pt,
  title=Box~\thetcbcounter: #2, #1}

\newcommand{\reals}{{\mathbb R}}
\newcommand{\dof}{\emph{dof}}
\newcounter{remark}[section]
\newcommand{\remark}{\noindent \textbf{Remark} \refstepcounter{remark} \textbf{\theremark} \;}




\definecolor{Sun}{rgb}{0.164,0.126,0.322}
\definecolor{Green}{rgb}{0,0.300,0.300}
\definecolor{Red}{rgb}{0.4,0,0}
\definecolor{Grey}{RGB}{105,105,105}
\definecolor{White}{rgb}{1,1,1}

% for blocks in Algorithm
\algblockdefx{Start}{End}[1]{\textbf{#1}}{\textbf{end}}

%without this, xelatex would not work with fontspec
\DeclareTextCommand{\nobreakspace}{T1}{\leavevmode\nobreak\ }
% \numberwithin{equation}{section}


% add multiple graphics path
\graphicspath{{./}} 

\makeatletter
\def\@author#1{\g@addto@macro\elsauthors{\normalsize%
    \def\baselinestretch{1}%
    \upshape\authorsep#1\unskip\textsuperscript{%
      \ifx\@fnmark\@empty\else\unskip\sep\@fnmark\let\sep=,\fi
      \ifx\@corref\@empty\else\unskip\sep\@corref\let\sep=,\fi
      }%
    \def\authorsep{\unskip,\space}%
    \global\let\@fnmark\@empty
    \global\let\@corref\@empty  %% Added
    \global\let\sep\@empty}%
    \@eadauthor={#1}
}
\makeatother
